Large-Scale Analysis of Framework-Specific Exceptions in Android Apps

Mobile apps have become ubiquitous. For app developers, it is a key priority to ensure their apps' correctness and reliability. However, many apps still suffer from occasional to frequent crashes, weakening their competitive edge. Large-scale, deep analyses of the characteristics of real-world app crashes can provide useful insights to guide developers, or help improve testing and analysis tools. However, such studies do not exist -- this paper fills this gap. Over a four-month long effort, we have collected 16,245 unique exception traces from 2,486 open-source Android apps, and observed that framework-specific exceptions account for the majority of these crashes. We then extensively investigated the 8,243 framework-specific exceptions (which took six person-months): (1) identifying their characteristics (e.g., manifestation locations, common fault categories), (2) evaluating their manifestation via state-of-the-art bug detection techniques, and (3) reviewing their fixes. Besides the insights they provide, these findings motivate and enable follow-up research on mobile apps, such as bug detection, fault localization and patch generation. In addition, to demonstrate the utility of our findings, we have optimized Stoat, a dynamic testing tool, and implemented ExLocator, an exception localization tool, for Android apps. Stoat is able to quickly uncover three previously-unknown, confirmed/fixed crashes in Gmail and Google+; ExLocator is capable of precisely locating the root causes of identified exceptions in real-world apps. Our substantial dataset is made publicly available to share with and benefit the community.

==> related_work.tex <==
\section{Related Work}
\label{sec:rel}

\noindent{\emph{\textbf{Empirical Study}}}. 
Researchers have conducted several empirical studies to investigate various aspects of Android, \eg, performance~\cite{Liu:ICSE2014}, fragmentation~\cite{Wei16}, resource usage~\cite{LiuWXC16,Liu16}, API stability~\cite{McDonnell13} and security~\cite{Enck11}.
Although there is some existing work~\cite{Hu11,Zaeem14,Coelho15} on analyzing Android bugs or exceptions, their goals are different: Coelho \etal~\cite{Coelho15} analyzed exception traces to investigate the bug hazards of exception-handling code (\eg, cross-type exception wrapping), and Zaeem \etal~\cite{Zaeem14} studied app bugs to study generation of testing oracles on a particular set of bug types. 
Hu \etal~\cite{Hu11} summarized some bug categories, but they only investigated 10 apps and the generality and completeness of their conclusions are unclear.
Other researchers study Android and Symbian OSes' failures~\cite{Maji10} and Windows Phone app crashes~\cite{Ravindranath14}.
Therefore, to our knowledge, we are the first to investigate Android app crashes, and give an in-depth analysis.

\noindent{\emph{\textbf{Crash Detection, Localization, and Fixing}}}.
Researchers have contributed a line of research~\cite{AnandNHY12,vanderMerwe2012,MachiryTN13,AzimN13,YangPX13,ChoiNS13,MahmoodMM14,Hao2014,
AmalfitanoFTTM15,MaoHJ16,stoat17} to detect app crashes, but have not investigated the root causes of them.
As for crash localization, Sinha \etal~\cite{Sinha09} combine dynamic analysis and static backward data-flow analysis to locate a subclass of runtime exceptions, \eg, \texttt{NullPointer}, \texttt{Arithmetic} exceptions, in \texttt{Java}.
Jiang \etal~\cite{Jiang10} develop a similar approach.
Mirzaei \etal~\cite{Mirzaei15} adopt a statistical fault localization technique~\cite{Jones05} to rank suspicious code that causes the crash. But the effectiveness is unclear.
CrashLocator~\cite{Wu14} uses control-flow analysis and slicing techniques to identify faulty functions via recovering the crash stack into a static call graph.  However, they can only locate faults at function level.
Gao \etal~\cite{GaoZWXZM15} use stack trace information to query Stack Overflow posts, and generate promising fixes for Android apps.
Instead, our exception localization tool identifies the root causes based on our understanding, which is more precise and effective.


